Percival: Making In-Browser Perceptual Ad Blocking Practical With Deep Learning

In this paper we present Percival, a browser-embedded, lightweight, deep learning-powered ad blocker. Percival embeds itself within the browser's image rendering pipeline, which makes it possible to intercept every image obtained during page execution and to perform blocking based on applying machine learning for image classification to flag potential ads. Our implementation inside both Chromium and Brave browsers shows only a minor rendering performance overhead of 4.55%, demonstrating the feasibility of deploying traditionally heavy models (i.e. deep neural networks) inside the critical path of the rendering engine of a browser. We show that our image-based ad blocker can replicate EasyList rules with an accuracy of 96.76%. To show the versatility of the Percival's approach we present case studies that demonstrate that Percival 1) does surprisingly well on ads in languages other than English; 2) Percival also performs well on blocking first-party Facebook ads, which have presented issues for other ad blockers. Percival proves that image-based perceptual ad blocking is an attractive complement to today's dominant approach of block lists

==> dups <==
#!/usr/bin/env perl
 
# Finds duplicate adjacent words.
 
use strict ;
 
my $DupCount = 0 ;
 
if (!@ARGV) {
  print "usage: dups <file> ...\n" ;
  exit ;
}
 
while (1) {
  my $FileName = shift @ARGV ;
 
  # Exit code = number of duplicates found.  
  exit $DupCount if (!$FileName) ;
 
  open FILE, $FileName or die $!; 
   
  my $LastWord = "" ;
  my $LineNum = 0 ;
   
  while (<FILE>) {
    chomp ;
 
    $LineNum ++ ;
     
    my @words = split (/(\W+)/) ;
     
    foreach my $word (@words) {
      # Skip spaces:
      next if $word =~ /^\s*$/ ;
 
      # Skip punctuation:
      if ($word =~ /^\W+$/) {
        $LastWord = "" ;
        next ;
      }
       
      # Found a dup? 
      if (lc($word) eq lc($LastWord)) {
        print "$FileName:$LineNum $word\n" ;
        $DupCount ++ ;
      } # Thanks to Sean Cronin for tip on case.
 
      # Mark this as the last word:
      $LastWord = $word ;
    }
  }
   
  close FILE ;
}


==> passive <==
#!/bin/bash
 
irregulars="awoken|\
been|born|beat|\
become|begun|bent|\
beset|bet|bid|\
bidden|bound|bitten|\
bled|blown|broken|\
bred|brought|broadcast|\
built|burnt|burst|\
bought|cast|caught|\
chosen|clung|come|\
cost|crept|cut|\
dealt|dug|dived|\
done|drawn|dreamt|\
driven|drunk|eaten|fallen|\
fed|felt|fought|found|\
fit|fled|flung|flown|\
forbidden|forgotten|\
foregone|forgiven|\
forsaken|frozen|\
gotten|given|gone|\
ground|grown|hung|\
heard|hidden|hit|\
held|hurt|kept|knelt|\
knit|known|laid|led|\
leapt|learnt|left|\
lent|let|lain|lighted|\
lost|made|meant|met|\
misspelt|mistaken|mown|\
overcome|overdone|overtaken|\
overthrown|paid|pled|proven|\
put|quit|read|rid|ridden|\
rung|risen|run|sawn|said|\
seen|sought|sold|sent|\
set|sewn|shaken|shaven|\
shorn|shed|shone|shod|\
shot|shown|shrunk|shut|\
sung|sunk|sat|slept|\
slain|slid|slung|slit|\
smitten|sown|spoken|sped|\
spent|spilt|spun|spit|\
split|spread|sprung|stood|\
stolen|stuck|stung|stunk|\
stridden|struck|strung|\
striven|sworn|swept|\
swollen|swum|swung|taken|\
taught|torn|told|thought|\
thrived|thrown|thrust|\
trodden|understood|upheld|\
upset|woken|worn|woven|\
wed|wept|wound|won|\
withheld|withstood|wrung|\
written"
 
if [ "$1" = "" ]; then
 echo "usage: `basename $0` <file> ..."
 exit
fi
 
egrep -n -i --color \
 "\\b(am|are|were|being|is|been|was|be)\
\\b[ ]*(\w+ed|($irregulars))\\b" $*
 
exit $?


==> weasel <==
#!/bin/bash
 
weasels="many|various|very|fairly|several|extremely\
|exceedingly|quite|remarkably|few|surprisingly\
|mostly|largely|huge|tiny|((are|is) a number)\
|excellent|interestingly|significantly\
|substantially|clearly|vast|relatively|completely"
 
wordfile=""
 
# Check for an alternate weasel file
if [ -f $HOME/etc/words/weasels ]; then
    wordfile="$HOME/etc/words/weasels"
fi
 
if [ -f $WORDSDIR/weasels ]; then
    wordfile="$WORDSDIR/weasels"
fi
 
if [ -f words/weasels ]; then
    wordfile="words/weasels"
fi
 
if [ ! "$wordfile" = "" ]; then
    weasels="xyzabc123";
    for w in `cat $wordfile`; do
        weasels="$weasels|$w"
    done
fi
 
 
if [ "$1" = "" ]; then
 echo "usage: `basename $0` <file> ..."
 exit
fi
 
egrep -i -n --color "\\b($weasels)\\b" $*
 
exit $?

